The average genus of oriented rational links with a given crossing number

In this paper, we enumerate the number of oriented rational knots and the number of oriented rational links with any given crossing number and minimum genus. This allows us to obtain a precise formula for the average minimal genus of oriented rational knots and links with any given crossing number.

==> genus_knot.dat.tex <==
n   $g_k$
4	1
5	1.5
6	1.6
7	1.857142857
8	2.095238095
9	2.375
10	2.588235294
11	2.846153846
12	3.085043988
13	3.34375
14	3.583882784
15	3.83777938
16	4.08350119
17	4.3359375
18	4.583382925
19	4.834572067
20	5.083347639
21	5.333984375
22	5.583337386
23	5.833653931
24	6.083334466
25	6.333496094
26	6.583333646
27	6.833414346
28	7.083333419
29	7.333374023
30	7.583333357
31	7.833353652
32	8.08333334
33	8.333343506
34	8.583333335
35	8.833338418
36	9.083333334
37	9.333335876
38	9.583333333
39	9.833334605
40	10.08333333
41	10.33333397
42	10.58333333
43	10.83333365
44	11.08333333
45	11.33333349
46	11.58333333
47	11.83333341
48	12.08333333
49	12.33333337
50	12.58333333
51	12.83333335

==> genus_link.dat.tex <==
n	g_l(D)
4	0.5
5	1
6	1
7	1.4
8	1.533333333
9	1.857142857
10	2.058823529
11	2.341176471
12	2.572192513
13	2.835777126
14	3.078321678
15	3.334065934
16	3.581037567
17	3.833546969
18	4.082255
19	4.333394369
20	4.582815664
21	4.8333505
22	5.083080873
23	5.333338102
24	5.583208942
25	5.833334645
26	6.083271658
27	6.333333691
28	6.583302641
29	6.83333343
30	7.083318027
31	7.333333359
32	7.583325691
33	7.83333334
34	8.083329665
35	8.333333335
36	8.583331425
37	8.833333334
38	9.083332379
39	9.333333333
40	9.583332856
41	9.833333333
42	10.08333309
43	10.33333333
44	10.58333321
45	10.83333333
46	11.08333327
47	11.33333333
48	11.5833333
49	11.83333333
50	12.08333332
51	12.33333333
